Outer Rotation Curve of the Galaxy with VERA I: Trigonometric parallax of IRAS 05168+3634

We report measurement of trigonometric parallax of IRAS 05168+3634 with VERA. The parallax is 0.532 +/- 0.053 mas, corresponding to a distance of 1.88+0.21/-0.17 kpc. This result is significantly smaller than the previous distance estimate of 6 kpc based on kinematic distance. This drastic change in the source distance revises not only physical parameters of IRAS 05168+3634, but also its location of the source, placing it in the Perseus arm rather than the Outer arm. We also measure proper motions of the source. A combination of the distance and the proper motions with systemic velocity yields rotation velocity ({\Theta}) of 227+9/-11 km s-1 at the source, assuming {\Theta}0 = 240 km s-1. Our result combined with previous VLBI results for six sources in the Perseus arm indicates that the sources rotate systematically slower than the Galactic rotation velocity at the LSR. In fact, we show observed disk peculiar motions averaged over the seven sources in the Perseus arm as (Umean, Vmean) = (11 +/- 3, -17 +/- 3) km s-1, indicating that these seven sources are systematically moving toward the Galactic center, and lag behind the Galactic rotation.

==> 00README.XXX.tex <==
nohypertex

